A Large-scale Investigation of Semantically Incompatible APIs behind Compatibility Issues in Android Apps

Application Programming Interface (API) incompatibility is a long-standing issue in Android application development. The rapid evolution of Android APIs results in a significant number of API additions, removals, and changes between adjacent versions. Unfortunately, this high frequency of alterations may lead to compatibility issues, often without adequate notification to developers regarding these changes. Although researchers have proposed some work on detecting compatibility issues caused by changes in API signatures, they often overlook compatibility issues stemming from sophisticated semantic changes. In response to this challenge, we conducted a large-scale discovery of incompatible APIs in the Android Open Source Project (AOSP) by leveraging static analysis and pre-trained Large Language Models (LLMs) across adjacent versions. We systematically formulate the problem and propose a unified framework to detect incompatible APIs, especially for semantic changes. It's worth highlighting that our approach achieves a 0.83 F1-score in identifying semantically incompatible APIs in the Android framework. Ultimately, our approach detects 5,481 incompatible APIs spanning from version 4 to version 33. We further demonstrate its effectiveness in supplementing the state-of-the-art methods in detecting a broader spectrum of compatibility issues (+92.3%) that have been previously overlooked.

==> 10_draft.tex <==
Here is an example of Different Return Value.
\begin{lstlisting}
// android.os.StrictMode.ThreadPolicy.Builder.permitUnbufferedIo
// Version 28
{
    return disable(DETECT_UNBUFFERED_IO);
}
// Version 29
{
    return disable(DETECT_THREAD_UNBUFFERED_IO);
}
\end{lstlisting}
Here is an example of Different Control Dependency.
\begin{lstlisting}
// android.os.Environment.isExternalStorageEmulated
// AOSP Version 27
{
    if (isStorageDisabled())
        return false;
    final File externalDir = sCurrentUser.getExternalDirs()[0];
    return isExternalStorageEmulated(externalDir);
}
// AOSP Version 28
{
    final File externalDir = sCurrentUser.getExternalDirs()[0];
    return isExternalStorageEmulated(externalDir);
}
\end{lstlisting}
Here is an example of Different Exception Handling.
\begin{lstlisting}
// android.app.usage.NetworkStatsManager.queryDetails
// AOSP Version 23
{
    NetworkTemplate template = createTemplate(networkType, subscriberId);
    if (template == null) {
        return null;
    }
    ...
}
// AOSP Version 24
{
    NetworkTemplate template;
    try {
        template = createTemplate(networkType, subscriberId);
    } catch (IllegalArgumentException e) {
        if (DBG)
            Log.e(TAG, "Cannot create template", e);
        return null;
    }
    ...
}
\end{lstlisting}


% examples for in-context learning
% <android.os.StrictMode.ThreadPolicy.Builder: Builder permitUnbufferedIo()>

==> backup.tex <==
\lili{Motivation: semantic changes, ROM differences}

%Android platform is an open-source software stack that allows developers to get access to the entire feature-set through framework APIs written in Java language. Such mechanism convenience users to build blocks to create Android apps by simplifying the usage of Android core system, including interacting with components and services. However, 
%Previous studies on the evolution of Android ecosystem have shown that the revision of platform APIs will lead to various compatibility issues. Li et al.\cite{li2018cid} claimed that various compatibility issues arise thanks to the evolution of Android framework APIs which would cause runtime crashes with error messages. On top of that, H. Huang et al.\cite{huang2018understanding} revealed \emph{callback compatibility issues} existing in Android framework API due to the update of Android framework. 



In the Android ecosystem, developers are allowed to declare the API level (\emph{minSdkVersion/maxSdkVersion/targetSdkVersion}) to uniquely specify the framework API version that suits most. These sdkVersions are designated to the minimum/max/target API Level for the app to run. However, in practice we discover that such settings are not always meet the requirements recommended by google. For example, we found that various apps in AndroZooOpen\cite{liu2020androzooopen} don’t clearly indicate \emph{minSdkVersion} and \emph{maxSdkVersion} in manifests. Indeed, if the \emph{minSdkVersion} is not declared, the system assumes a default value of "1", which indicates that this app is compatible with all versions of Android. Nevertheless, if APIs above level x(x>1) are involved and this app occasionally installed on a system with an API level less than x, this application would crash during runtime when these unavailable APIs are invoked. Thus, if  \emph{minSdkVersion} is not set, any Android operating system might contain runtime compatibility issues due to the abuse of unsuitable framework APIs.

A few previous works have explored API compatibility issues in Android system\cite{li2018cid,wei2016taming,mutchler2016target,zhang2015compatibility,ham2011mobile,huang2018understanding}.
\lili{motivation: (1) API needs unit test, (2) better for crowdsourced testing.}

Overall, we make the following key contributions:
\begin{itemize}
	\item 
    We propose an automatic Unit Test generation tool to discover API compatibility issues that are not exposed to the state-of-the-art static and dynamic analysis tools in the Android ecosystem. We also packaged all these generated test cases into an APK which would output API compatibility-related issues during its execution on different devices.   
	\item 
	We design and implement a prototype tool \tool{} for detecting compatibility issues by generating executable unit test cases from the bytecode of thousands of real-world Android apps. To that end, these test cases can be executed directly on different kinds of Android platforms to identify API compatibility issues.
	 
	\item 
	We evaluated \tool{} on a set of real Android devices and report on the API compatibility issues that \tool{} identifies and inspects. We further investigate the useful of \tool{} \xiaoyu{todo}

\end{itemize}

\subsection{API Caller Instance Inference (ACII)} ACII is responsible for identifying the caller instance of the target Android APIs and generating the executable call sequence from the caller to the target API.
%To that end, we implement the ACII module for extracting all the accessible Android APIs from app bytecode and then perform a sequence of static analyses for API usage mining, including call graph analysis, forward data-flow analysis, inter-procedural backward data-flow analysis, etc. Figure \ref{fig:ACII} shows the working process of Module ACII, which is carried out in the following three steps:
It contains the following three steps, as illustrated in Figure \ref{fig:ACII}:
\begin{enumerate}[label=(\roman*)]
\item Locating Android Framework APIs
\item Building API Usage Call Graphs
\item Constructing API Call Sequences
\end{enumerate}

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/ACII.pdf}
	\caption{The working process of Module ACII.}
    \label{fig:ACII}
\end{figure}

\textbf{Locating Android Framework APIs.} Given an Android app, \tool{} firstly extract the Dalvik Bytecode from the APK, which is then transformed into Jimple intermediate representation \cite{vallee2010soot}. \tool{} then retrieves target Android APIs that have been invoked by sweeping over the Jimple code. The located Android APIs are passed to the next module for further analysis.

%\textbf{Locating Android Framework APIs.} \tool{} firstly retrieves all Android framework API invocations by analysing its bytecode of a given Android APK. To achieve this, we first summarize the two basic kinds of method invocation in Java programming language:\emph{instance methods} and \emph{class (or static) methods}. In general, the major difference between them are:
%1. Instance methods require an instance before they can be invoked, whereas static methods are the methods that can be called without creating an object of class.
%2. While Instance methods are invoked by using object reference, static methods can be invoked by using class reference
%3. While static methods will only exist as a single copy for a class, instance methods exist as multiple copies depending on the number of instances created for that class.

%To elaborate the different instructions of these two methods, we provide code examples in Table~\ref{tab:Category_API_Type} for each method. To generate an executable unit test for instance method, we must mining the actual class of the instance and usage of it from the source code. In this example, ACII would conduct a backward data-flow analyses to locate both the definition statement for \$r5 and its related sequences of API calls. In addition, referring to static method, ACII would only require to record the method signature of the API for unit test generation. In the code example, as long as we extract the exact API signature(\emph{<android.text.TextUtils: boolean equals(java.lang.CharSequence, java.lang.CharSequence)>}) of the API, it is possible for \tool{} to generate the corresponding unit test directly. To that end, in the following part we further explain the backward tracking data-flow analysis to identify the instance.



%the actual class of \$r11 is defined in line 12, which is \emph{\$r11 = (android.net.ConnectivityManager) \$r10;}.
%Since this definition statement contains another object which remains unknown(\$r10), we need to further identify the actual class of \$r10. To that end, \tool{} conduct a backward tracking process to mining the whole API usage. When there is a filed involved in the backward tracking flow, our data-flow analysis will keep tracking the exact value of this field as it is necessary to generate a complete executable unit test. For example, \tool{} would keep tracking when field statement \emph{\$r0.<com.comment.one.h.a: android.content.Context n>} is reached. Besides, when there is a user-defined method involved in the backward tracking flow, \tool{} will further keep tracking the returned variables of this method (all variables are involved if there are several return statements). Apart from that, when there is a parameter statement involved, the backward tracking process will keep working to identify the actual class from all its callers. Finally, the backward tracking analysis will terminate if System APIs are reached or there is no unknown variable in the current statement.

%\textbf{Building API Usage CG} The ACII module performs a \textbf{backward data-flow analysis} to generate minimum API usage context for all involved framework APIs. Indeed, the actual class of instance can not be easily identified directly in source code. A sequence of invocation statements and constructing objects can be involved from the initiative code to the target API. Besides, the statements can be instantiate in other methods and convey to the object via callee's returned values or caller's parameter values. Therefore, we propose a backward data-flow analysis to mine the API usage, including \textbf{inter-procedural} process which is aware of \textbf{constructor methods} and \textbf{field assignments}.

%In the example of Listing~\ref{code:Code_Example_API_Caller_Instance}, the actual class of \$r11 is defined in line 12, which is \emph{\$r11 = (android.net.ConnectivityManager) \$r10;}. Since this definition statement contains another object which remains unknown(\$r10), we need to further identify the actual class of \$r10. To that end, \tool{} conduct a backward tracking process to mining the whole API usage. When there is a filed involved in the backward tracking flow, our data-flow analysis will keep tracking the exact value of this field as it is necessary to generate a complete executable unit test. For example, \tool{} would keep tracking when field statement \emph{\$r0.<com.comment.one.h.a: android.content.Context n>} is reached. Besides, when there is a user-defined method involved in the backward tracking flow, \tool{} will further keep tracking the returned variables of this method (all variables are involved if there are several return statements). Apart from that, when there is a parameter statement involved, the backward tracking process will keep working to identify the actual class from all its callers. Finally, the backward tracking analysis will terminate if System APIs are reached or there is no unknown variable in the current statement.




%Given a sequence of invocation statements and constructing objects in the call path, the ACII module can retrieve accurate API usage. Since these statements are collected by backward analysis, we now need to reverse them to generate a executable code block for target API testing. On top of that, considering the UI-related APIs, some unique resourceId would involve in the minimum context which prevents such code block from execution. Thus, the ACII module better to weed out these UI-related APIs to avoid false positive results. What's more, if reflection calls are involved in the minimum context, we can't successfully resolve its actual class, which we plan to optimize by integrating reflection augment tool DroidRA\cite{li2016droidra} into this work in the future.

% \begin{lstlisting}[
% caption={Code Example of API Caller Instance Inference.},
% label=code:Code_Example_API_Caller_Instance,
% firstnumber=1]
% public final class com.comment.one.h.a
% {
% public android.content.Context n;

% public final void a(android.content.Context, int, int, java.lang.String, java.lang.String, com.comment.one.main.CallBackListener)
% {
%  $r0 := @this: com.comment.one.h.a;
%  $r1 := @parameter0: android.content.Context;
%  $r0.<com.comment.one.h.a: android.content.Context n> = $r1;
%  $r8 = $r0.<com.comment.one.h.a: android.content.Context n>;
%  $r10 = $r8.<android.content.Context: java.lang.Object getSystemService(java.lang.String)>("connectivity");
%  $r11 = (android.net.ConnectivityManager) $r10;
%  //API need to be tested
%  $r12 = $r11.<android.net.ConnectivityManager: android.net.NetworkInfo getActiveNetworkInfo()>();
% }}
% \end{lstlisting}

\begin{itemize}

\item \textbf{Missing Android specific objects.}
add Activity architecture
  For those cases where we need to launch Activity before API invocation, \tool{} using soot to program an Activity architecture. Take \ref{code:Code_Example_Activity_Architecture} for an example, the Activity architecture lies in line 4,7,8,14-17, where we leverage \emph{ActivityTestRule.getActivity()} to get the reference of the activity and the Activity is assigned during the initial creation of the activity(line 14-17).
  Regarding the \emph{MyActivity} in line 15, it is a basic Activity  


  \item Field substitute. 
  If user-defined filed is involved in unit test, \tool{} will traverse all the methods in its declare class to pinpoint the identification statement for this field. Then \tool{} would replace the original filed with the new identified object. To that end, we can successfully eliminate compatible errors caused by original fields. 
 
  \item Inject constructor 
  When the backward data-flow analysis encounter a JNewExpr, it is necessary to figure out its init method because the unit test is incompatible becasue of lacking its corresponding construct method. Thus, \tool{} will go a further step to detect the corresponding constructor and then inject it after the JNewExpr. 
  
  \item add Activity architecture
  For those cases where we need to launch Activity before API invocation, \tool{} using soot to program an Activity architecture. Take \ref{code:Code_Example_Activity_Architecture} for an example, the Activity architecture lies in line 4,7,8,14-17, where we leverage \emph{ActivityTestRule.getActivity()} to get the reference of the activity and the Activity is assigned during the initial creation of the activity(line 14-17).
  Regarding the \emph{MyActivity} in line 15, it is a basic Activity  
  
  \item add Static architecture
  For those framework API that was described with "static", we can't invoke it directly in unit test because Junit doesn't support adding annotation(@Test) on static method. Thus, we use soot to create a static architecture for this scenario. \ref{code:Code_Example_Static_Architecture} is the code example, the static architecture lies in line 7-10, and it will invoke another static method in line 3, which contains the content of the API usage of a specific API.
  
 

\end{itemize}

\textbf{Construct Activity And Static Architecture}
\begin{lstlisting}[
caption={Code Example of Activity Architecture.},
label=code:Code_Example_Activity_Architecture,
firstnumber=1]
@RunWith(AndroidJUnit4.class)
public class TestCase_com_tux_client__137805151 {
   @Rule
   public ActivityTestRule mActivityRule;
   @Test
   public void testCase() throws Exception {
      ActivityTestRule var1 = this.mActivityRule;
      Activity var2 = var1.getActivity();
      Intent var3 = var2.getIntent();
      Bundle var4 = var3.getBundleExtra("CertInfo");
      SslCertificate var5 = SslCertificate.restoreState(var4);
      String var6 = var5.getValidNotAfter();
   }
   public TestCase_com_tux_client__137805151() {
      ActivityTestRule var1 = new ActivityTestRule(MyActivity.class);
      this.mActivityRule = var1;
   }
}
\end{lstlisting}


\lili{field replacement. Find a code example}


\begin{lstlisting}[
caption={Test Case of field replacement},
label=code:Test_Case_Field_Replacement,
firstnumber=1]
@RunWith(AndroidJUnit4.class)
public class TestCase_905a4f82bc194334a046afa9bf29eed7__2022256821 {
 @Test
 public void testCase() throws Exception {
     Context var1 = InstrumentationRegistry.getTargetContext();
     Object var2 = var1.getSystemService("connectivity");
     ConnectivityManager var3 = (ConnectivityManager)var2;
     NetworkInfo var4 = var3.getActiveNetworkInfo();
 }
}
\end{lstlisting}


\begin{lstlisting}[
caption={Code example of field replacement. The code snippet is extracted from app \emph{com.odgq.dfoqg.iruwue.apk}.},
label=code:Code_Example_Field_Replacement,
firstnumber=1]
public final class com.comment.one.h.a {
 public android.content.Context n;
    
 public final void a(android.content.Context, int, int, java.lang.String, java.lang.String, com.comment.one.main.CallBackListener) {
  $r1 := @parameter0: android.content.Context;
  $r0.<com.comment.one.h.a: android.content.Context n> = $r1;
  $r8 = $r0.<com.comment.one.h.a: android.content.Context n>;
  $r10 = virtualinvoke $r8.<android.content.Context: java.lang.Object  getSystemService(java.lang.String)>("connectivity");
  $r11 = (android.net.ConnectivityManager) $r10;
  $r12 = virtualinvoke $r11.<android.net.ConnectivityManager:android.net.NetworkInfo  getActiveNetworkInfo()>();
}}
\end{lstlisting}


\begin{description}
  \setlength\itemsep{0.05em}

\item[RQ1] To what extent can \tool{} generate executable unit test cases for Android APIs?

Notes:
exclude UI-resourceID
exclude broadcast

API 29 (1000) -> successfully execution rate

\item[RQ2] When increasing the number of Android apps for mining API usages, can \tool{} generate unit test cases covering more Android APIs?
\xiao{also report the time spent on generating \& executing the test cases.}
Notes:
1000 (RQ1) -> 1900 (distinct)/3000 APIs (with successful test cases) -> 10000 test cases can be successfully executed
1000(RQ1) + 1000 (new) -> 2200 (distinct) / 3000 APIs, 15000 test cases
1000(RQ1) + 1000 (new) -> 2500 (distinct) / 3000 APIs, 20000 test cases

1000(distinct, all), 2000 (distinct, all), 3000 (distinct, all)

-> successfully executed APIs

USED APIs

API usages -> successful rate (the more number of test cases, the more likely we will generate a valuable test cases).


RQ2's results: 40\% unsuccessful API (all test cases) -> incompatible APIs


\item[RQ3] How effective is \tool{} in discovering API-induced Compatibility Issues? 

Notes:
API 21->29 (1000)

TYPE1, TYPE2, TYPE1+TYPE2

%Device-specific
\end{description}
